XNOR-FORMER: Learning Accurate Approximations in Long Speech Transformers

Transformers are among the state of the art for many tasks in speech, vision, and natural language processing, among others. Self-attentions, which are crucial contributors to this performance have quadratic computational complexity, which makes training on longer input sequences challenging. Prior work has produced state-of-the-art transformer variants with linear attention, however, current models sacrifice performance to achieve efficient implementations. In this work, we develop a novel linear transformer by examining the properties of the key-query product within self-attentions. Our model outperforms state of the art approaches on speech recognition and speech summarization, resulting in 1 % absolute WER improvement on the Librispeech-100 speech recognition benchmark and a new INTERVIEW speech recognition benchmark, and 5 points on ROUGE for summarization with How2.

==> sections/intro.backup.tex <==
Transformers are among the state of the art for many tasks in speech, natural language processing and vision, among other fields. Transformers achieve their exceptional generalizability in part due to multi-head self-attention, represented as a softmax normalization of the dot product between a ``query'' and ``key''. However, this attention mechanism requires the explicit computation of an $N \times N $ attention matrix (where $N$ is the length of the input), resulting in quadratic time and space complexity.

As a result, it becomes challenging to operate on longer input sequences with such transformers on modern GPUs and TPUs, and training such models from scratch is time and labor intensive. Therefore, the input is partitioned into chunks, and each chunk is compressed into  a compact representation\cite{dai-etal-2019-transformer,Rae2019CompressiveTransformer} that serves as context for future chunks. However, training over smaller chunks loses often important context from previous chunks, and context passing requires additional storage. This results in a quadratic asymptotic complexity. 

% attention mechanisms, leading to linear approximations to multihead self-attention. 

% Over time, more complex tasks that were earlier performed by a cascade pipeline have begun to be addressed by these transformer variants that can handle long input sequences. Speech summarization of videos , document level language modelling, and <insert CV task here> are examples of such tasks which needed the input data to be segmented into smaller chunks to enable processing. 

% ADDED by bhiksha
The computational challenges arise from the computational formulation of self-attention, which has the form $softmax(cQK^\top)V$, where $Q$, $K$ and $V$ are the query, key and value matrices, respectively, and $c$ is some scaling term.  The bottleneck arises from $softmax(QK^\top)$: both $Q$ and $K$ have one dimension equal to $N$, as a result of which $QK^\top$ requires $O(N^2)$ computation. This cannot be factored, since the softmax operates on the \emph{product}, which must necessarily be computed before the softmax is applied.

Recently, many works have had success in developing attention mechanisms that approximate the standard self-attention in linear time and space complexity.  Solutions to this challenge include using low-rank approximations of the softmax output\cite{wang2020linformer,xiong2021nystromformer}, local and global attentions\cite{Zaheer2020BigBird,Beltagy2020Longformer,ainslie-etal-2020-etc}, and the kernel trick for linear attentions \cite{zhen2022cosformer,katharopoulos_et_al_2020,choromanski2021rethinking}. Pattern based methods \cite{dai-etal-2019-transformer,Beltagy2020Longformer,Zaheer2020BigBird,Rae2019CompressiveTransformer} or sparsity based methods \cite{xiong2021nystromformer,wang2020linformer} can operate on sequences upto a maximum length, and have the computational complexity of approximating standard self-attentions. Linear transformers\cite{zhen2022cosformer,katharopoulos_et_al_2020}, on the other hand, can operate on long sequences, and require constant time for each auto-regressive inference step. However, current linear transformers still have significant performance degradations compared to the standard self-attention.


 In this paper, we attempt to bridge this gap by developing the \emph{XNOR self-attention} and correspondingly, the \emph{XNOR-transformer}. Our work falls into the pool of work on linear transformers that use the kernel trick to compute self-attentions in linear time. Rather than computing the matrix product $QK^T$, and consequently, $softmax(QK^T)V$, linear transformers formulate $softmax(QK^T)=f(Q)g(K^T)$, where $f(\cdot)$ and $g(\cdot)$ represent kernel functions. Further, they use the associativity property of matrix multiplication to re-order the operations, i.e., $[f(Q)g(K^T)]V = f(Q)[g(K^T)V] $. This allows the key-value product to be pre-computed once, leading to a time complexity that depends on the length of the query $N$. The choice of kernel function is important to satisfy the known properties of attention weights, and approximate full self-attention with arbitrary precision.  


We begin by identifying two important properties of attention weights- (1) they are always non-negative, and (2) attention weights sum to unity. A kernel function that retains these properties is the softmax kernel, which produces Markov matrices. The product of Markov matrices is known to be Markov, i.e., the resulting attention weights are guaranteed to be non-negative and sum to unity. Empirically, we find that the softmax kernel by itself does not yield the best performance. 

Consider a two-dimensional softmax function, which is equivalent to a sigmoid. We find that the sigmoid of a product can be approximated as the sum of the products of the component sigmoids and their complements. We extend this principle to the softmax kernel, and arrive at the formulation for XNOR self-attention. Transformer self-attentions are position agnostic, and positional information has been found to be useful within the self-attention\cite{zhen2022cosformer,su2021roformer,dai-etal-2019-transformer}. However standard mechanisms are unsuitable for linear transformers since they require the explicit computation of attention weights. Inspired by \cite{zhen2022cosformer,su2021roformer}, we explore the use of rotational and cosine relative positional embeddings and integrate them with the proposed XNOR-former. 


Most prior work examines long sequence transformers on image and text-based tasks, while we conduct experiments on speech recognition and summarization.  Speech recognition and summarization tasks are different from text-based tasks in the following ways: (a) speech input signals are generally longer, by a factor of 10-100, (b) in speech signals, adjacent frames are often correlated, unlike natural language where adjacent tokens can be less so. 

Our proposed approach outperforms prior kernel methods on two speech recognition benchmarks and end-to-end speech summarization, while demonstrating competitive performance on the Long Range Arena \cite{tay2021long} benchmark. 


This paper is organized as follows: Section \ref{sec:proposed_approach} describes the proposed approach, Section \ref{sec:related_work} discusses related work, Section \ref{sec:setup} explains design and evaluation of our experiments, Section \ref{sec:results} details our experimental results and ablation studies. 

==> sections/method.orig.tex <==
\label{sec:proposed_approach}
\subsection{Standard Self-Attention}

Consider an input sequence $X$ of length $N$. The self-attention weights $O$ are then computed using three unique projections of the input sequence- entitled the query Q, key K and value V. Multi-head self-attention \cite{vaswani2017} can be formulated with key $ K=XW_K \in  \mathbb{R}^{N \times d}$, query $Q=XW_Q \in  \mathbb{R}^{N \times d}$, softmax operator $Sm()$ and value $V=XW_V \in  \mathbb{R}^{N \times d}$. The output of this self-attention $\mathcal{O} \in \mathbb{R}^{N \times d} = [ \mathcal{O}_1 \mathcal{O}_2 \cdots \mathcal{O}_N ]^T$ is given by Equation \ref{equation:vaswani_attn}.

\begin{equation}
    \label{equation:vaswani_attn}
    \mathcal{O} = \sum_{i=1}^N Sm\Big(\frac{QK^T}{\sqrt{d}}\Big).V
\end{equation}


To obtain a more general form( see Equation \ref{equation:general_attn}), the softmax can be replaced by a similarity measure $S(Q_i,K_j)= Sm(\frac{Q_iK_j}{\sqrt{d}})$, and the softmax normalization can be replaced by a normalization step.

\begin{equation}
            \label{equation:general_attn}
    \mathcal{O}_i = \sum_{i=1}^N \frac{S(Q_i,K_j)}{\sum_{j} S(Q_i,K_j)}.V_j
\end{equation}


This self-attention necessitates the computation of the matrix $QK^T$, which results in a quadratic complexity for the attention with respect to the input length $N$ since each $\mathcal{O}_i$ computation requires the softmax normalization of an $N \times N $ matrix. Therefore, it is not viable to compute on long input sequences. Next, we examine linear self-attention mechanisms that use the kernel trick and matrix product associativity to replace the softmax product. 



\subsection{Linear Transformers}

To extend this approach for long input sequences, the dot product based softmax similarity is replaced by a product in kernel space, i.e.,  $S(\mathcal{Q},\mathcal{K}) = \phi(\mathcal{Q})\phi(\mathcal{K})^T$. Using the associative law of matrix multiplication, we can multiply the key $\phi(\mathcal{K})^T$ and value $V$, and reorder the matrix multiplication to have linear time complexity. The output $O_i$ is given in Equation \ref{equation:general_linear_attn}.

\begin{equation}
    \label{equation:general_linear_attn}
    \mathcal{O}_i = \sum_{i=1}^N \frac{\phi(Q_i)(\phi(K_j)V_j)}{\sum_{j} \phi(Q_i)\phi(K_j)}
\end{equation}

Prior works have used approximations with Gaussian Kernels\cite{choromanski2021rethinking}, ELU based kernels\cite{katharopoulos_et_al_2020}, and ReLU kernels\cite{zhen2022cosformer}. Though prior approaches have had success in tasks, empirically, they are accompanied by undesirable performance reductions. 
We examine the most basic instance of a softmax in 2 dimensions, the sigmoid to derive approximations for the softmax term in self-attention. We also investigate methods to incorporate relative positional information within the self-attention. 

\subsection{Softmax Kernel Attention}

The attention matrix has two properties: (1) it is non-negative, and (2) the attention weights add up to unity. In order to obtain a linear transformer that fulfills these constraints, we can consider the choice of a softmax kernel, i.e., $\phi=Sm()$. The softmax kernel results in Markov matrices for every example, and the product of two Markov matrices is always non-negative. Consider $o^TA = o^T, o^TB=o^T$ , i.e., both have columns that sum to 1. Then, $o^TAB= o^TB=o^T$. Therefore, the product of two Markov matrices is also Markov, fulfilling the attention weight sum property.  

\begin{equation}
    \mathcal{O}_i = \sum_{i=1}^N \frac{Sm(Q_i)(Sm(K_j)V_j)}{\sum_{j} Sm(Q_i)(Sm(K_j) }
        \label{equation:softmax_attn}
\end{equation}


\subsection{Examining the Sigmoid of the Product}

The simplest instance of a softmax would be for a 2 dimensional projection, where the softmax reduces to a sigmoid activation. Under this constraint, the  similarity measure $S(XY^T)=Sm(XY^T)$ can be represented as $\sigma(XY)$, where $\sigma()$ and $Sm()$ represent the sigmoid and softmax activations respectively. 


Now, we attempt to find a function that is able to approximate the sigmoid of the product $XY^T$ without explicitly needing to compute the product. That is, we want to find $f\colon \mathcal{R} \to \mathcal{R} \mid \sigma(XY)= f(\sigma(X),\sigma(Y))$. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/sigmoidxyplot.png}
    \caption{Plot of $\sigma(XY)$ for X=-1000:0.05:1000,Y=-1000:0.05:100. The resulting function has high values when both X and Y have the same sign}
    \label{fig:sigmoid_xy_plot}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/errorxy.png}
    \caption{Plot of $E(X,Y) = \sigma(XY)- \sigma(X)\sigma(Y)-(1-\sigma(X)(1-\sigma(Y)$ for X=-1000:0.05:1000,Y=-1000:0.05:100. The error function demonstrates that the XNOR-formulation is a reasonable approximation for the sigmoid product $\sigma(XY)$}
    \label{fig:error_xy_plot}
\end{figure}

Figure \ref{fig:sigmoid_xy_plot} shows the plot of the function $\sigma(XY)$ over values of values of x and y between -100 and 100. We observe that this function appears like an extension of the XNOR function, which produces the highest outputs when the signs of x and y are matched. We verify this observation by plotting the error function $ E(X,Y) = \sigma(XY)-\sigma(X)\sigma(Y) $ in Figure \ref{fig:error_xy_plot}. 

Equation \ref{equation:sigmoid_xnor_factorization}  defines the X-NOR approximation of the sigmoid of the product of two random variables where $\sigma' = 1- \sigma$, the complement of the sigmoid operator

\begin{equation}
\label{equation:sigmoid_xnor_factorization}
\sigma(XY)=\sigma(X)\sigma(Y)+\sigma'(X)\sigma'(Y)
\end{equation}

% We observe that this formulation, though it minimizes the error, does not lead to zero error. Therefore, we insert learnable weights $w_1$, and $w_2$ on the XNOR formulation to help recover lost information as follows:
% \begin{equation}
%     \sigma(XY)=w_1\sigma(X)\sigma(Y)+ w_2(1-\sigma(X))(1-\sigma(Y))
% \end{equation}

\subsection{X-NOR Self-Attention}
\label{sec:xnor_selfattn}
Drawing from the X-NOR approximation of the sigmoid, we can now extend this to approximate the softmax product in Equation \ref{equation:softmax_xnor_factorization} where $Sm$ represents the softmax operator and $Sm' = 1- Sm$ represents its complement:
\begin{equation}
    \label{equation:softmax_xnor_factorization}
    S(Q_i,K_j) = Sm(Q_i)Sm(K_j)+ Sm'(Q_i)Sm'(K_j)
\end{equation}

We note that the softmax activation and the sigmoid are not equivalent for projection dimensions that are not equal to 2, but demonstrate empirically that the proposed X-NOR formulation improves model performance over merely using a softmax kernel $\phi= Sm()$. The resulting XNOR factorization allows self-attention to be computed in linear time and space complexity. 


The two terms in the XNOR formulation represent correlations between the query and key, and their complements. In order to make the formulation more flexible, interpretable and accurate, we weight these parameters differently for each instance of the XNOR self-attention with learnable scalar weights $w_1$ and $w_2$. This results in the Weighted XNOR (W-XNOR) formulation as follows:

\begin{equation}
\begin{split}
\mathcal{O}_i & = w_1\sum_{i=1}^N \frac{Sm(Q_i)(Sm(Kq_j)V_j)}{\sum_{j} Sm(Q_i)Sm(K_j)}) \\ & + w_2 \sum_{i=1}^N \frac{Sm'(Q_i)(Sm'(K_j)V_j)}{\sum_{j} Sm'(Q_i)Sm'(K_j)})
\end{split}
    \label{equation:softmax_wxnor}
\end{equation}

Equation \ref{equation:softmax_wxnor} represents the weighted X-NOR formulation. Next, we will examine how to integrate positional information into the attention formulation. Note that the two terms in the formulation can be computed in parallel.



\subsection{Positional Encodings}

Self-attention mechanisms are inherently position agnostic, and attention computations are performed independently in parallel for every time step. Therefore, transformer self-attentions require explicit positional embeddings within the attention mechanism to incorporate awareness of the relative position $i-j$ or absolute positions $i,j$ within the sequence. Relative positional embeddings were demonstrated to outperform absolute embeddings in \cite{dai-etal-2019-transformer,shaw-etal-2018-self} Learnable relative positional encodings, introduced in \cite{dai-etal-2019-transformer} rely on computing the full attention matrix, and hence cannot be used with linear attentions since the full attention weights are not computed explicitly. 

To embed positional information into the XNOR self-attention, or in general for linear transformers that use the kernel trick, candidate encodings must have two characteristics:
\begin{enumerate}
    \item The resulting attention output $O_i$ should depend on relative position $i-j$, i.e., $P(Q_i,K_j)=f(i-j)$
    \item The positional encoding should be factorable into the kernel outputs of the key and query respectively, i.e., $P(Q_i,K_j)=g(i)h(j)$
\end{enumerate}

Let $T_1=\sum_{i=1}^N \frac{Sm(Q_i)(Sm(Kq_j)V_j)}{\sum_{j} Sm(Q_i)Sm(K_j)},T_2= \sum_{i=1}^N \frac{Sm'(Q_i)(Sm'(K_j)V_j)}{\sum_{j} Sm'(Q_i)Sm'(K_j)}$. The positional encoding can then be multiplied with the output as shown in Equation \ref{equation:softmax_wxnor_pos} 
\begin{equation}
\label{equation:softmax_wxnor_pos}
\mathcal{O}_i & = w_1 T_1 P(Q_i,K_j) + w_2 T_2P(Q_i,K_j)
\end{equation}




Based on prior work, we adopt two formulations for the positional encoding: a cosine form \cite{zhen2022cosformer}, and rotational positional encodings \cite{su2021roformer}. The cosine positional encodings are realized using Ptolemy's theorem as defined in Equation \ref{equation:cos_pos}. M is the maximum sequence length in the batch of examples to ensure that the the $cos(x)$ is computed within $0 < x < \pi/2 $
\begin{equation}
\label{equation:cos_pos}
\begin{split}
    P(Q_i,K_j) &= cos\Big(\frac{\pi}{2} * \frac{(i-j)}{M}\Big) \\
    &= cos\Big(\frac{\pi i}{2*M}\Big)cos\Big(\frac{\pi j}{2*M}\Big)\\
    &+sin\Big(\frac{\pi i}{2*M}\Big)sin\Big(\frac{\pi j}{2*M}\Big)
\end{split}
\end{equation}

Rotational positional encoding encode absolute positional information within rotation matrices. The product of rotation matrices encodes relative information. Equation \ref{equation:rot_pos} defines the rotational positional embedding, where $\mathbb{R}^d_{\Theta,j}$ is a d-dimensional rotation matrix that encodes the absolute position $j$.  We refer interested readers to \cite{su2021roformer} for a complete mathematical treatment.

\begin{equation}
\label{equation:rot_pos}
    P(Q_i,K_j) = \mathbb{R}^d_{\Theta,n-m} = \mathbb{R}^d_{\Theta,m}\mathbb{R}^d_{\Theta,n}
\end{equation}

% \textbf{ADD DETAILS IN HERE IF THERE IS SPACE AT THE END}





% Cosine self-attention\cite{zhen2022cosformer} was introduced to derive a linear cost replacement of quadratic self-attention without approximating the softmax function. Using a ReLU kernel as a replacement for the softmax ensures non-negativity of the attention scores. The authors further propose a cosine based re-weighting scheme that stabilizes attention weights by amplifying local correlations. The proposed cosine re-weighting results in the similarity metric $ S(\mathcal{Q}_i,\mathcal{K}_j) =\text{ReLU}(\mathcal{Q}_i)\text{ReLU}(\mathcal{K}_j) \text{cos}(\dfrac{i-j}{N})$. Let $K_j^{sin} = \text{ReLU}(K_j) sin(\frac{j\pi}{2N})$, $K_j^{cos}\text{ = ReLU}(K_j) cos(\frac{j\pi}{2N})$, $Q_i^{sin}\text{ = ReLU}(Q_i) sin(\frac{i\pi}{2N})$, and $Q_i^{cos}\text{ = ReLU}(Q_i)sin(\frac{i\pi}{2N})$. The resulting output is then:
% % \begin{equation}
% %     S(\mathcal{Q}_i,\mathcal{K}_j) = ReLU(\mathcal{Q})ReLU(\mathcal{K})^T
% %     %cos\Big(\dfrac{i-j}{M}\Big) 
% % \end{equation}
% % \begin{equation}
% %     \mathcal{O}_i =  \dfrac{ \sum_{j=1}^N ReLU(K_j)V_j}{ ReLU(Q_i) \sum_{j=1}^N ReLU(K_j)}
% % \end{equation}
% \begin{equation}
%     \mathcal{O}_i =  \dfrac{ \sum_{j=1}^N Q^{cos}_i ((K_j^{cos})^T V_j) + \sum_{j=1}^N Q^{sin}_i ((K_j^{sin})^T V_j)  }{ \sum_{j=1}^N Q^{cos}_i (K_j^{cos})^T + \sum_{j=1}^N Q^{sin}_i (K_j^{sin})^T}
% \end{equation}

% The cosine re-weighting also functions as a relative positional embedding for the attention computation, and has been shown to improve performance on bidirectional fine-tuning tasks \cite{zhen2022cosformer}.



==> sections/related.tex <==
\label{sec:related_work}

In this section, we describe related work in building efficient transformers. 

\textbf{Partial Attention or Pattern Based Methods:} Some works utilize sparsity or attention patterns to use only a portion of the input to approximate full attention.  \cite{dai-etal-2019-transformer} use segment wise recurrence within transformer self attentions to provide longer context (~900 words). \cite{Rae2019CompressiveTransformer} compresses the segment level contexts and provides them as additional input to enable a longer context than Transformer-XL. Other works have focused on making the self-attentions sparse to reduce computational complexity. The Reformer\cite{kitaev2019reformer} uses Locality Sensitive Hashing to compute localized self attentions in O(nlogn), but the large constant term makes the complexity difference significant for very long sequences. Longformer \cite{Beltagy2020Longformer} uses different attention patterns for each layer and window based dilated self-attentions, and Big Bird\cite{Zaheer2020BigBird} uses a combination of sliding window, global and random attentions to reduce the complexity of self-attentions. These methods don't perform as well as the standard self-attention, and the main issue with this approach is the computational overhead that arises from auxiliary operations like gather, scatter, slicing and concatenation, which are not inexpensive on modern hardware.

\cite{wang2020linformer} uses  using the kernel trick and Johnson–Lindenstrauss lemma to approximate the low-rank self attention to arbitrary precision. \cite{xiong2021nystromformer} uses the Nystrom method to approximate the low rank self-attention matrix. However, such pattern based methods can operate only on sequences upto a maximum length, and the  computational complexity of approximating to arbitrary precision increases with the sequence length. 


\textbf{Sparse Approximations and Linear Transformers}:  Another line of important work linearizes the computation of self-attentions and using matrix associativity to obtain self-attentions within linear time and space complexity.The kernel trick is employed to approximate the softmax attention, with ELU kernels\cite{katharopoulos_et_al_2020}, FAVOR+ kernels \cite{choromanski2021rethinking,chen-2021-permuteformer}, ReLU kernels \cite{zhen2022cosformer}, and ReLU squared kernels \cite{hua2022flash}. However such methods appear to do significantly worse than our proposed kernel (see Table \ref{tab:librispeech_100}). 
Linear attention is particularly appealing since it can be implemented in constant time for each inference step. Hence, in this work, we attempt to develop a kernel function and positional encoding that improve the performance of such linear transformers. 


